On the Limitations and Capabilities of Position Embeddings for Length Generalization

In Transformers, Position Embeddings (PEs) significantly influence Length Generalization (LG) performance, yet their fundamental role remains unclear. In this work, we investigate the limitations and capabilities of PEs in achieving LG. We theoretically analyze PEs in Position-Only Linear Attentions (POLAs), introducing Linear Representation Complexity (LRC) to characterize when PEs enable LG. Our analysis shows that PEs do not expand computational capabilities but structure learned computations across positions. Extending to practical Transformers, we propose Sequential Representation Complexity (SRC) and conjecture that LG is possible if and only if SRC remains invariant across scales. We support this hypothesis with empirical evidence in various reasoning tasks. To enhance LG, we introduce Scale Hint, allowing flexible instance scaling, and a Learning-Based Position Embedding framework that automatically learns positional relations. Our work provides theoretical insights and practical strategies for improving LG in Transformers.

==> sections/biographies.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biographies/yangchen.png}}]
{Yang Chen} is a Ph.D. student at Peking University. His research interests include reasoning, learning theory, and optimization. Chen received his B.S. in Computer Science from Peking University. His work has been published at top-tier conferences such as ICML and NeurIPS.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biographies/yitaoliang.png}}]
{Yitao Liang} is an assistant professor and Boya Fellow at Peking University. He obtained his Ph.D. degree in Computer Science from UCLA, advised by Prof. Guy Van den Broeck. His research interests span knowledge reasoning, machine learning and AI agents. His work has received recognition from top AI conferences; for example, the best-paper honorable mention from AAMAS 2016, the best paper from RL for Real Life workshop in ICML 2019, a best paper runner-up from the LLD workshop in NeurIPS 2017, a best paper from the TEACH workshop in ICML2023. He regularly serves as area chairs and senior area chairs in top venues e.g., NeurIPS, ICML.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biographies/zhouchenlin.png}}]
{Zhouchen Lin} (M'00-SM'08-F'18) received the Ph.D. degree in applied mathematics from Peking University in 2000. He is currently a Boya Special Professor with the State Key Laboratory of General Artificial Intelligence, School of Intelligence Science and Technology, Peking University. His research interests include machine learning and numerical optimization. He has published over 350 technical papers, collecting more than 40,000 Google Scholar citations. He has been a Program co-Chair of ICPR 2022, Area Chairs of ACML, ACCV, CVPR, ICCV, NIPS/NeurIPS, AAAI, IJCAI, ICLR, and ICML and Senior Area Chairs of ICML, NeurIPS, CVPR and ICLR for many times. He was an Associate Editor of the IEEE Transactions on Pattern Analysis and Machine Intelligence and currently is an associate editor of the International Journal of Computer Vision and Optimization Methods and Software. He is a Fellow of the IAPR, the IEEE, the AAIA, and the CSIG.
\end{IEEEbiography}
